Triangle-free 2-matchings

We consider the problem of finding a maximum size triangle-free $2$-matching in a graph $G=(V,E)$. A (simple) $2$-matching is any subset of the edges such that each vertex is incident to at most two edges from the subset. The first polynomial time algorithm for this problem was given by Hartvigsen in 1984 in his PhD thesis and its improved version has been recently published in a journal. We present a different, significantly simpler algorithm with a relatively short proof of correctness. Our algorithm with running time $O(|V||E|)$ is additionally faster than the one by Hartvigsen having running time $O(|V|^3|E|^2)$. It has been proven before that for any triangle-free $2$-matching $M$ which is not maximum the graph contains an $M$-augmenting path, whose application to $M$ results in a bigger triangle-free $2$-matching. A new observation is that the search for an augmenting path $P$ can be restricted to so-called {\em amenable} paths that go through any triangle $t$ contained in $P\cup M$ a limited number of times. Amenable paths can be characterised with the aid of {\em half-edges}. A {\em half-edge} of edge $e$ is, informally speaking, a half of $e$ containing exactly one of its endpoints. Each half-edge serves also as a {\em hinge} - a connector between one pair of edges on an alternating path. To find an amenable augmenting path we thus dynamically remove and re-add half-edges to forbid or allow some edges to be followed by certain others. The existence of amenable augmenting paths follows from our decomposition theorem for triangle-free $2$-matchings. This decomposition theorem is largely the same as the decomposition from versions 1-6 of this paper and is moreover simpler and stronger than the one given by Kobayashi and Noguchi.

==> 2match.tex <==

\subsection{Maximum matchings and $2$-matchings}

Before proceeding further with the description of an algorithm for a maximum triangle-free $2$-matching, let us explain some properties of  algorithms for finding, respectively, a maximum matching and a maximum $2$-matching (that may contain triangles).

Let us start with a standard matching $M$. Suppose that $M$ is a matching in $G$ and $s$ is a vertex unmatched in $M$. We review an algorithm for finding an $M$-augmenting path starting at $s$. The algorithm maintains a structure $S$ that at the beginning consists only of the vertex $s$ and further on a vertex $v$
is contained in $S$ only if $S$ contains an $M$-alternating path from $s$ to $v$.
Let $\mathcal{E}(S)$ denote the set $\{v \in S: S$ contains an even-length $M$-alternating path from $s$ to $v \}$.  Vertices of $\mathcal{E}(S)$ are called {\bf \em even}.
Let $\mathcal{O}(S)$ denote the set $\{v \in S: S$ contains an odd-length $M$-alternating path from $s$ to $v \}$. %Vertices of $\mathcal{O}(S)$ are called {\bf \em odd} or $\mathcal{O}$-vertices.
If a vertex $v$ belongs to $\mathcal{O}(S) \cap \mathcal{E}(S)$, then $S$ contains a blossom $B$, which means that $S$ contains  an even-length $M$-alternating path $P$ from $s$ to a vertex $b$, called the {\bf \em base} of $B$ and an odd-length
$M$-alternating path $B=(b,v_1, v_2, \ldots, v_{2k-1}, v_{2k}, b)$ such that $P$ and $B$ are vertex-disjoint except for the vertex $b$ and $v \in \{v_1, \ldots, v_{2k}\}$. %(In the case of  $b$-matchings $B$ and $P$ are vertex-disjoint except for the vertex $b$.) 
A blossom $B$ is said to be {\bf \em even} if its base $b$ belongs to $\mathcal{E}(S)$. It can be proved that each blossom $B$ that is not a singleton, i.e., contains more than one vertex, is even throughout the algorithm constructing $S$. Any blossom may contain subblossoms. A blossom $B$ that is not contained in any other blossom is called {\bf \em outer}. In many algorithms dealing with similar structures, a blossom is  treated as one vertex and shrunk. For every vertex $v \in \mathcal{E}(S)$, the structure $S$ contains exactly one even-length alternating path $P_v$ starting at $s$ and ending at $v$. 
If $P_v$ uses at least one edge of a blossom $B$, then all edges of $P_v \cap B$ form one subpath $P'$ of $P_v$ such that
 one endpoint of $P'$ is the base of $B$. In the paper structure $S$,  blossoms as well as $\bar{S}$, explained below, are defined in the same way as in \cite{Gabow17} Section 3.2. The algorithms in the paper also maintain $\bar{S}$, the subgraph $S$ with blossoms contracted. $\bar{S}$ is a tree. It is also an ''alternating tree''. Any path from a vertex in $S$ to $s$ is alternating. 
More information about blossoms can also be found for example in Lov\'asz and Plummer~\cite{LovaszPlummer2009} or in \cite{Schrijver2003}.



We say that an edge $(u, v)$ is incident to a blossom $B$ if  $u$ belongs to $B$.  
We say that an edge $(u,v)$ such that $u$ belongs to a blossom $B$ is {\bf \em $S$-augmenting} if $v \notin B$ and either $v \notin S$ or $v \in \mathcal{E}(S)$.
After the addition of such an edge  to $S$, $S$ either contains some new vertex $v$ or $S$ contains a new blossom - a new blossom is formed by a fundamental cycle $C$ in $\bar{S} \cup (u,v)$ and contracted. (Note that $C$ forms  an alternating path in $bar{S}$ but not an alternating cycle.)
Note that we do not add $(u,v)$ if $v \notin B$ and $v \in \mathcal{O}(S) \setminus \mathcal{E}(S)$.




\begin{algorithm}[H]
\begin{algorithmic}[1]

	
	\State Let $s$ be an unmatched vertex in $M$. Set $S \leftarrow \{s\}$.  
	Assume that each vertex $v$ is contained in an unprocessed blossom containing only $v$.
	
	
	
	\While {$ \exists$ an even unprocessed blossom  in $S$} 
	\State $B \ \leftarrow \ $ an even unprocessed blossom in $S$
	 
	\For {each  $S$-augmenting edge $(u,v)$ incident to $B$ such that $u \in B$}
	
	\If {$ v \notin S$}
	  \State add $(u,v)$ to $S$
		\If {$v$ is matched in $M$}
		 \State add $(v, M(v))$ to $S$
		\EndIf
	\Else 
	  \State add $(u,v)$ to $S$
		\State form a new blossom $B'$, which contains $B$ and $(u,v)$ and leave loop {\em for}
		
	
	
	\EndIf
	\EndFor
	\State call $B$ processed
	\EndWhile
\end{algorithmic}
\caption{Computing a set of $M$-alternating paths starting at an unmatched vertex $s$.}
\label{algmaxM}
\end{algorithm}


Suppose now that $M$ is a $2$-matching and $s$ an unsaturated vertex in $M$. 
Finding an $M$-augmenting path in $G$ starting at $s$ may be reduced to finding  an $M'$-augmenting path in $G'$ starting at $s$.
%When building $S$ that contains $M'$-alternating paths starting at $S$ we only add those edges of $G'$ that increase the set $\mathcal{E}(S)$ (this is consistent with the majority of algorithms computing maximum (standard) matchings).
To make the presentation clearer, we extend $G_2$ and $G'$ so that $s$ is the only unmatched vertex in $M'$  in the following manner.
For every unmatched in $M'$ vertex $v_i$ different from $s$ we add a new vertex $v^M_i$ and a new edge $(v_i, v^M_i)$ to $M'$. The set of all such new vertices is denoted as $V_s$.
Thus we get an obvious correspondence between $M$-augmenting paths in $G$ starting in $s$ and even-length alternating paths beginning in $s$ in $G'$ and ending in vertices of $V_s$.
\begin{observation}
An even length alternating path from $s$ to $v^M_i$ in $G'$ corresponds to an $M$-augmenting path from $s$ to $v$ in $G$.
\end{observation}


Each blossom $B$ that is not a singleton, i.e., contains more than one vertex, is considered to be an even blossom. Observe that the base of any non-singleton blossom is connected  
to $s$ by an even-length alternating path in $G_2$ - see an example in Figure \ref{blossomG2G}.

\begin{figure}[h]
\centering{\includegraphics[scale=0.8]{blossomG2G.pdf}}
\caption{\small On the left, a blossom $B$ in $G$ on vertices $a,b,c$ and base in $a$ and on the right, its counterpart in $G_2$ with base in $x^a_{sa}$.}
 \label{blossomG2G}
\end{figure}

When we are interested in finding a $2$-matching we may ignore edges in $G'$ whose addition would only result in adding vertices of $X$ and not $V'$ to $S$.
For example, if $c_1 \in \mathcal{O}(S), d_1, b_1 \in \mathcal{E}(S)$  and $S$  contains $(c_1, d_1) \in M'$ but none of  the edges $(b_1, x^b_{bc}), (x^b_{bc},  x^c_{bc}), (x^c_{bc},c_1) \in E'$, then while processing $b_1$ we would extend $S$ to the edges $(b_1, x^b_{bc}), (x^b_{bc},  x^c_{bc})$. We can, however, see that the addition of these edges
to $S$ does not imply that we have identified any further vertex of $V'$ reachable via an $M'$-alternating path from $s$. For this reason,  we extend $S$ by edges in $M'$ or by $3$-edge-paths in $G'$ corresponding to edges in $G$.
%To this end we define segments. A segment is defined as either one half-edge or a $3$-edge-path in $G'$ containing two half-edges of the same edge $e$ in $G$ (such $e$ cannot thus belong to $M$) and an edge of the form $(x^u_{uv}, x^v_{uv})$.  If the endpoints of a path forming a segment are $u_i, v_j$, then the segment is denoted as $seg=(u_i, v_j)$.
For any two vertices $u_i, v_j$ (such that $u_i$ is a copy of $u \in G$ and $v_j$ is a copy of $v \in G$) we say that $seg(u_i, v_j)$ is a {\bf \em segment} of $G_2$  if $(u,v) \in E\setminus M$. %We say that a segment $seg(u_i, v_j)$ is incident to a blossom $B$ if  $u_i$ belongs to $B$.  

Let $seg(u_i, v_j)$ be a segment and $B$ a blossom in $S$ such that $u_i \in B, v_j \notin B$.
We define this segment as {\bf \em $S$-augmenting} if 
  $v_j \notin \mathcal{O}(S) \setminus \mathcal{E}(S)$ (i.e. $v_j \in \mathcal{E}(S)$ or $v_j \notin S$),
and  $x^v_{uv} \notin \mathcal{O}(S) \setminus \mathcal{E}(S)$, and in the case when $x^u_{uv} \in B$, one hinge $(u_i, x^u_{uv})$ of the segment already belongs to $B$.



After the addition of such a segment  to $S$, %together with $H(seg)$,
 $S$ satisfies at least one of the following:(i)  one new vertex $v' \in V' \cup V_s$ belongs to $\mathcal{E}(S)$ or (ii) $S$ contains a new blossom.

Thus an algorithm that finds all vertices of $V' \cup V_s$ reachable from $s$ via an even-length alternating path can be stated as follows.

\begin{algorithm}[H]
\begin{algorithmic}[1]

	
	\State Let $s$ be an unmatched vertex in $M'$. Set $S \leftarrow \{s\}$.  
	Assume that each vertex $v$ is contained in an unprocessed blossom containing only $v$.
	
	
	
	\While {$ \exists$ an even unprocessed blossom  in $S$} 
	\State $B \ \leftarrow \ $ an even unprocessed blossom in $S$
	 
	\For {each  $S$-augmenting segment $seg=(u_i,v_j)$ incident to $B$ such that $u_i \in B$}
	
	
		\State add $seg (u_i,v_j)$ to $S$
		
	\If {$ v_j \notin B$}
	  \State add $(v_j, M'(v_j))$ to $S$
		
	\Else 
	   
		\State form a new blossom $B'$, which contains $B$ and $seg(u_i,v_j)$ and leave loop {\em for}
		
	
	
	\EndIf
	
	
	
	
	
	%\EndIf
	\EndFor
	\State call $B$ processed
	\EndWhile
\end{algorithmic}
\caption{Computing a set of $M$-augmenting paths starting at an unsaturated vertex $s$.}
\label{algmax2M}
\end{algorithm}


\begin{figure}
\centering{\includegraphics[scale=0.85]{superfluous.pdf}}
\caption{On the left there is a graph $G$ and on the right its representation as $G'$. If $S$ already contains the edges $(s,a)$ and $(a,c)$, then we do not need add to $S$ also the edges $(s,b), (b,c)$.}
 \label{superfluous}
\end{figure}

The main goal of the algorithm above is, however, to compute a set of $M$-augmenting paths starting at an unsaturated vertex $s$ instead of all vertices of $V' \cup V_s$ reachable from $s$ via an even-length alternating path.
In the case of $2$-matchings, as opposed to matchings, we can  notice that if $v_i \in \mathcal{E}(S)$, then we may sometimes ignore extensions to $S$, which would result only in that the other copy  of $v$ would belong to $\mathcal{E}(S)$. An example is shown in Figure \ref{superfluous}.
For this reason we introduce the notion of alternating $s$-reachability.
We say that two subgraphs $H_1, H_2$ of $G_2$ have the same {\bf \em alternating $s$-reachability} if for every vertex $v \in V \cup V_s$ it holds that $H_1$ contains an even length alternating path from $s$ to some copy of $v$ if and only if $H_2$ does. 
Let $G_2[S]$ denote all edges of $G_2$ considered so far while building $S$ in the algorithm.
Then, we may notice that at the end of each iteration of {\em while}-loop it holds that $S$ has the same alternating $s$-reachability as $G_2[S]$.

We say that an edge or segment of $G_2$ is {\bf \em superfluous} for $S$ if its addition to $S$ does not increase its alternating $s$-reachability. 
%Thus, any segment $seg(u_i, v_j)$ such that (i) $u_i \in \mathcal{E}(S)$ and  $v_j \in \mathcal{O}(S)$ or (ii) $u_i, v_j$ belong to the same blossom in $S$, is superfluous.
%Also, as stated in Fact \ref{altE}, a segment $seg(u_i, w_j)$ incident to a  blossom $B$ in $S$  such that: (i) $u_i \in B$, (ii) $w_j \notin S$ and (iii) $M(w_j)=bro(v_i)$, is superfluous. However, a segment that is superfluous for $S$ at some point of the algorithm may cease to be such at a later point. For example a segment $seg(u_i, v_j)$ of type (i)
%may later become one that satisfies: $u_i, v_j \in \mathcal{E}(S)$ and $u_i, v_j$ are not contained in the same blossom.
We say that an edge or segment of $G_2$ is {\bf \em lastingly superfluous} for $S$ if it is superfluous and remains superfluous for $S$ at every later point of the algorithm.
 







